Multi-task Learning for Universal Sentence Embeddings: A Thorough Evaluation using Transfer and Auxiliary Tasks

Learning distributed sentence representations is one of the key challenges in natural language processing. Previous work demonstrated that a recurrent neural network (RNNs) based sentence encoder trained on a large collection of annotated natural language inference data, is efficient in the transfer learning to facilitate other related tasks. In this paper, we show that joint learning of multiple tasks results in better generalizable sentence representations by conducting extensive experiments and analysis comparing the multi-task and single-task learned sentence encoders. The quantitative analysis using auxiliary tasks show that multi-task learning helps to embed better semantic information in the sentence representations compared to single-task learning. In addition, we compare multi-task sentence encoders with contextualized word representations and show that combining both of them can further boost the performance of transfer learning.

==> table/table6.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[t]
\centering
\begin{tabular}{l@{\hskip 0.3in} c@{\hskip 0.3in} c@{\hskip 0.3in} c@{\hskip 0.3in} c@{\hskip 0.3in} c@{\hskip 0.3in} c@{}}
\hline
\multirow{2}{*}{Model Type} & \multicolumn{3}{c}{ROCStories} & \multicolumn{3}{c}{VIST}  \\ 
& PM & LSR & PMR & PM & LSR & PMR \\
\hline
\multicolumn{7}{l}{Sentence representation learning from single-task} \\ 
%\hline
BiLSTM-Max (SNLI)    & 75.45 & \textbf{75.60} & \textbf{18.87} & 68.74 & 69.88 & 9.01 \\ 
BiLSTM-Max (AllNLI)  & \textbf{75.92} & \textbf{75.60} & 18.17 &	\textbf{69.58} & \textbf{70.43} & \textbf{9.67} \\
\hline
\multicolumn{7}{l}{Sentence representation learning from three-tasks (DupQuD, SNLI and Multi-NLI)} \\
Shared Private & 71.98 & 73.98 & 15.66 & 67.36 & 69.52 & 8.92 \\
Adversarial Shared Private & 70.30 & 72.85 & 14.11 & 65.94 & 68.40 & 7.46 \\
\hline
\end{tabular}
\caption{Sentence reordering results for the best two single-task and multi-task learning settings. Bold-faced values denote the best results across the board.}
\label{table:sent_ord}
\end{table*}

==> table/table7.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[t]
\centering
% \resizebox{\linewidth}{!}{%
\begin{tabular}{l@{\hskip 0.05in} c@{\hskip 0.05in} c@{\hskip 0.05in} c@{\hskip 0.05in} c@{\hskip 0.05in} c@{\hskip 0.05in} c@{\hskip 0.05in} c@{}}
\hline
Model Type  & \begin{tabular}{@{}c@{}} Sent. \\ Length \end{tabular}  & \begin{tabular}{@{}c@{}} PP in \\ Syn. Parse \end{tabular} & Adjectives & Adverbs  & \begin{tabular}{@{}c@{}} Proper \\ Nouns \end{tabular}  & \begin{tabular}{@{}c@{}} Possessive \\ pronoun \end{tabular}  & \begin{tabular}{@{}c@{}} Cardinal \\ Number \end{tabular}  \\ 
\hline
\multicolumn{8}{l}{Sentence representation learning from single-task} \\
%\hline
BiLSTM-Max (on SNLI)    & 11.86 & 95.06	& 85.23 & 79.72 & 93.78 & 94.42 & 95.51 \\ 
BiLSTM-Max (on DupQuD)    & 12.56 & 93.92 & 86.85 & 77.69 & 95.14 & 93.25 & 95.59  \\ 
BiLSTM-Max (on Multi-NLI)   & 8.56 & 94.95 & 86.88	& \textbf{83.32}	& 94.06 & 96.30 & 96.89 \\
BiLSTM-Max (on AllNLI)   & 10.32 & 95.37 & 86.91 & 82.98 & 93.94 & 96.27 & 95.14 \\
\hline
\multicolumn{8}{l}{Shared-Private (trained on DupQuD, SNLI, and Multi-NLI)}  \\ 
Private Encoder (on DupQuD) & 13.44 & 93.91 & 83.61 & 76.05 & 94.35 & 90.73 & 94.36 \\
Private Encoder (on SNLI) &  12.34 & 93.83 & 84.66 & 76.47 & 94.16 & 93.46 & 94.69 \\
Private Encoder (on Multi-NLI) &  9.80 & \underline{95.37} & 87.36 & \underline{81.97} & 94.07 & \underline{\textbf{96.98}} & \underline{\textbf{97.10}}    \\
Shared Encoder &  11.17 & 94.41 & 86.83 & 81.30 & 94.90 & 93.05 & 95.36   \\
Combined Encoder  & \underline{7.24} & 95.03 & \underline{\textbf{88.10}} & 81.91 & \underline{95.24} & 95.48 & 96.75 \\
\hline
\multicolumn{8}{l}{Adversarial Shared-Private (trained on DupQuD, SNLI, and Multi-NLI)}  \\ 
Private Encoder (on DupQuD) & 13.44 & 94.50 & 85.52 & 72.72 & 94.20 & 91.98 & 94.55 \\
Private Encoder (on SNLI) & 12.34 & 95.02 & 86.18 & 77.70 & 93.59 & 93.61 & 94.17 \\
Private Encoder (on Multi-NLI) & 9.80 & 94.17 & 86.80 & 80.94 & 93.87 & \underline{96.03} & \underline{96.53}   \\
Shared Encoder & 9.73 & 93.20 & 85.94 & 79.60 & 94.56  & 87.51 & 94.69  \\
Combined Encoder & \underline{\textbf{7.16}} & \underline{\textbf{96.13}} & \underline{87.05} & \underline{81.59} & \underline{\textbf{95.66}} & 94.52 & 96.49 \\
\hline
\end{tabular}
% }
\caption{Auxiliary task results for the best two single-task and multi-task learning settings trained on different combinations of DupQuD, SNLI and Multi-NLI datasets. 
We use \emph{mean square error} as evaluation metric for sentence length prediction and \emph{F1} score for other tasks.
Underlined values indicate the best performance among different encoders of the shared-private models trained on the same set of tasks.
Bold-faced values denote the best results across the board.}
\label{table:aux_full_comparison}
\end{table*}

==> table/table9.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[t]
\centering
\begin{tabular}{l@{\hskip 0.3in} c@{\hskip 0.3in} c@{\hskip 0.3in} c@{\hskip 0.3in} c@{\hskip 0.3in} c@{\hskip 0.3in} c@{}}
\hline
\multirow{2}{*}{Model Type} & \multicolumn{3}{c}{ROCStories} & \multicolumn{3}{c}{VIST}  \\ 
& PM & LSR & PMR & PM & LSR & PMR \\
\hline
\multicolumn{7}{l}{Sentence representation learning from single-task} \\ 
%\hline
BiLSTM-Max (on SNLI)    & 75.45 & \textbf{75.60} & \textbf{18.87} & 68.74 & 69.88 & 9.01 \\ 
BiLSTM-Max (on DupQuD)   & 74.54 & 74.36 & 16.52 & 68.11 & 69.50 & 8.25 \\
BiLSTM-Max (on Multi-NLI)  & 74.04 & 74.74 & 17.53 & 68.13 & 69.88 & \textbf{9.77} \\
BiLSTM-Max (on AllNLI)  & \textbf{75.92} & \textbf{75.60} & 18.17 & \textbf{69.58} & \textbf{70.43} & 9.67 \\
\hline
\multicolumn{7}{l}{Shared-Private (trained on DupQuD, SNLI, and Multi-NLI)} \\
Private Encoder (on DupQuD) & 71.29 & 72.97 & 14.11 & 66.66 & 68.93 & 8.09 \\
Private Encoder (on SNLI) & \underline{73.91} & \underline{74.42} & \underline{16.09} & 67.73 & 69.40 & 8.72 \\
Private Encoder (on Multi-NLI) & 73.59 & 74.25 & 15.39 & \underline{68.40} & \underline{69.60} & \underline{8.92} \\
Shared Encoder & 71.98 & 73.98 & 15.66 & 67.36 & 69.52 & \underline{8.92} \\
% Combined Encoder & - & - & - & - & - & - \\
\hline
\multicolumn{7}{l}{Adversarial Shared-Private (trained on DupQuD, SNLI, and Multi-NLI)} \\
Private Encoder (on DupQuD) & 70.80 & 72.56 & 13.31 & 66.22 & 68.78 & 8.11 \\
Private Encoder (on SNLI) & 71.32 & 73.36 & 15.07 & 67.15 & 69.40 & 8.43 \\
Private Encoder (on Multi-NLI) & \underline{73.68} & \underline{74.85} & \underline{17.37} & \underline{68.06} & \underline{69.88} & \underline{8.80} \\
Shared Encoder & 70.30 & 72.85 & 14.11 & 65.94 & 68.40 & 7.46 \\
% Combined Encoder & - & - & - & - & - & - \\
\hline
\end{tabular}
\caption{Sentence ordering results for the best two single-task and multi-task learning settings. Underlined values indicate the best performance among different encoders of the shared-private models trained on the same set of tasks. Bold-faced values denote the best results across the board.
Due to the structure of the sentence ordering model, it is not feasible to conduct experiment on the combined encoder, so we skipped it.}
\label{table:sem_eval}
\end{table*}
